Aerial Base Station Positioning and Power Control for Securing Communications: A Deep Q-Network Approach

The unmanned aerial vehicle (UAV) is one of the technological breakthroughs that supports a variety of services, including communications. UAV will play a critical role in enhancing the physical layer security of wireless networks. This paper defines the problem of eavesdropping on the link between the ground user and the UAV, which serves as an aerial base station (ABS). The reinforcement learning algorithms Q-learning and deep Q-network (DQN) are proposed for optimizing the position of the ABS and the transmission power to enhance the data rate of the ground user. This increases the secrecy capacity without the system knowing the location of the eavesdropper. Simulation results show fast convergence and the highest secrecy capacity of the proposed DQN compared to Q-learning and baseline approaches.

==> include/related.tex <==
\textcolor{red}{It is good practice to have a separate section. Where space is limited, it can be included in the intro or other parts. Also we need to compare our results and conclusions to those from recent related works, those that apply, later in the paper.}

==> include/result2.tex <==
In this section, we analyze the performance of the proposed DQN-based UAV positioning and power control scheme in this paper for optimizing the secrecy capacity of the ground legitimate user in the presence of an eavesdropping attack. 

The simulation scenario consists of a single antenna ground UE, ABS mounted on an the UAV, and a single antenna malicious node that is performing a passive eavesdropping attack on the UL transmission initiated at the UE towards the ABS. The simulation scenario is shown in Fig.~\ref{fig:system}. The UE and the eavesdropper will be randomly distributed within a 2D area that has a $L_x$ length and a $L_y$ width. The ABS will be launched at random location with a fixed altitude and equipped with an omnidirectional antenna to facilitate the communication links with the served ground users. 

The simulation parameter and the hyperparameters for the proposed DQN solution are given in Table.~\ref{tab:parameters}. In particular, the training and target DNN networks consist of $4$ \hl{Why 4?} layers where each DNN contains two fully connected \hl{hidden} layers with $24$ and $32$ neurons, respectively. Each DNN has $3$ neurons at the input layer and $12$ neurons at the output layer, corresponding to the number of states \hl{(3)} and possible actions \hl{(12)}. \textcolor{red}{Have you explained what those states and actions are?}
The simulator %environment described in this paper is simulated in the 
is implemented in Python, using the PyTorch to train a DQN. %, while the illustration of the results has been performed using Matlab. 

In the evaluation of the performance of our proposed DQN algorithm, we are comparing the obtained secrecy capacity via the DQN against the same metric resultant from employing the Q-learning, greedy policy, and randomized states algorithms. 
The random scheme select the next position and power action at each time slot randomly, whereas the greedy policy assign the next action based on the highest Q-value \hl{continuously}. 
\begin{table}[t]
%\fontsize{12}{10}\selectfont
\fontsize{4}{8}\selectfont
\centering
\caption{Simulation parameters.}
\label{tab:parameters}
\resizebox{0.35\textwidth}{!}
{%
\begin{tabular}{|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Simulation  parameter}\end{tabular}     & \textbf{Value}                              \\ \hline
\begin{tabular}[c]{@{}c@{}}(L$_x$, L$_y$)\end{tabular} & (10, 10) m  \\ \hline
%\begin{tabular}[c]{@{}c@{}}L_y\end{tabular} & 10 m   \\ \hline
\begin{tabular}[c]{@{}c@{}} Number of episodes\end{tabular} & 9 $\times$ 10$^{4}$ \\ \hline
\begin{tabular}[c]{@{}c@{}} Number time slots per episode\end{tabular} &  200 \\ \hline
\begin{tabular}[c]{@{}c@{}} Learning rate\end{tabular} &  10$^{-6}$ \\ \hline
\begin{tabular}[c]{@{}c@{}} Discount factor\end{tabular} & 0.9 \\ \hline
%Noise variance                                                     & 10^{\text{-12} }       \\ \hline
%\begin{tabular}[c]{@{}c@{}}
%SNR at the reference point\end{tabular}                                                      & 90 dB       \\ \hline
%\begin{tabular}[c]{@{}c@{}}dx    \end{tabular}        & 20 m                               \\ \hline
%M                                                          & 5 users                              \\ \hline
%\begin{tabular}[c]{@{}c@{}} Number of DNN layers\end{tabular} & 4 \\ \hline
%\begin{tabular}[c]{@{}c@{}} Number of NN nodes\end{tabular} &  \\ \hline
\begin{tabular}[c]{@{}c@{}} Replay memory size\end{tabular} & 500 entries \\ \hline
\begin{tabular}[c]{@{}c@{}} Batch size\end{tabular} & 50 \\ \hline
\begin{tabular}[c]{@{}c@{}} Update rate of target network\end{tabular} & 10 \\ \hline
% Bandwidth                                                          & 10 MHz                              \\ \hline
\end{tabular}%
}
\vspace{-5mm}
\end{table}
    \begin{figure*}
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{{figures/Reward.eps}}
    \caption{The reward}
    \label{fig:Reward}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/Distance.eps}
    \caption{The distance}
    \label{fig:Distance}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/Power.eps}
    \caption{The power}
    \label{fig:PW}
  \end{subfigure}
  \caption{The reward, distance and power convergence of the DQN, Q-learning and other base line techniques.}\label{fig:animals}
\end{figure*}

 
Figure.~\ref{fig:Secrecy} illustrates the obtained secrecy capacity for the DQN compared to the other %benchmarking 
techniques over the number of episodes. %AS it can be noted, 
The proposed DQN algorithm enhances the episode secrecy capacity by as much as 40\%, 10\%, and 5\% when compared to the randomized states, greedy policy, and the Q-learning, respectively. According to Figure.~\ref{fig:Secrecy}, the performance of the DQN reaches a relatively stable secrecy capacity value after $1 \times 10^4$ episodes. On the other hand, the convergence of Q-learning occurs after $5 \times 10^4$ episodes. This proves the superiority of the DQN regarding the speed of convergence. %\hl{explain why accepted or remove rest of the sentence:} with accepted secrecy capacity performance over the other techniques.
%   \begin{figure}[H]
%      \centering
%      \includegraphics[width=0.45\textwidth]{figures/Secrecy.eps}
%      \caption{Secrecy.}
%      %\vspace{-5mm}
%      \label{fig:Secrecy}
%  \end{figure}

Since the secrecy capacity optimization problem relies on the location of the ABS and the transmission power, it is critical to study the convergence of these two parameters for a better understanding of the secrecy capacity performance. Figures~\ref{fig:Distance} and~\ref{fig:PW} illustrate the convergence of the UAV positioning and the transmission power over the number of episodes, respectively. Comparing the converged position of the ABS and transmission power for the DQN and Q-learning, we can see that both techniques have reached the same ABS position, however there is a slight increase of the converged transmission power of the DQN over the converged Q-learning transmission power. This difference %in the converged transmission power 
is the main explanation behind the difference in the obtained secrecy capacity levels presented in Fig.~\ref{fig:Secrecy}. Moreover, the zero secrecy capacity of the randomized states approach %given that both of the greedy and random approaches have converged to the same position from Fig.~\ref{fig:Distance} is resultant 
results from low transmission power value shown in Fig.~\ref{fig:PW}. Note that the ABS position converges to the same as with the greedy algorithm.

%   \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.45\textwidth]{figures/Distance.eps}
%      \caption{Distance.}
%      %\vspace{-5mm}
%      \label{fig:Distance}
%  \end{figure}
%  \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.45\textwidth]{figures/Power.eps}
%      \caption{Power.}
%      %\vspace{-5mm}
%      \label{fig:PW}
%  \end{figure}
%   \begin{figure}[t]
%      \centering
%      \includegraphics[width=0.45\textwidth]{figures/Reward.eps}
%      \caption{Reward.}
%      %\vspace{-5mm}
%      \label{fig:Reward}
%  \end{figure}
Figure.~\ref{fig:Reward} shows our reward function that is defined as the legitimate UL capacity between the ground UE and the ABS without taking into consideration the eavesdropping capacity for the proposed DQN and other techniques. The illustrated reward functions inform that the proposed solution in this paper has the fastest convergence rate with higher capacity. On the other hand, the performance of the Q-learning is sufficient, but takes longer to converge because of the nature of the problem that has a large number of states. 
%  \begin{figure*}
%         \centering
%         \begin{subfigure}[b]{0.33\textwidth}
%             \centering
%             \includegraphics[width=\textwidth]{figures/Secrecy.eps}
%             \caption[Network2]%
%             {{\small Network 1}}    
%             \label{fig:mean and std of net14}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.33\textwidth}  
%             \centering 
%             \includegraphics[width=\textwidth]{figures/Distance.eps}
%             \caption[]%
%             {{\small Network 2}}    
%             \label{fig:mean and std of net24}
%         \end{subfigure}
%         \vskip\baselineskip
%         \begin{subfigure}[b]{0.33\textwidth}   
%             \centering 
%             \includegraphics[width=\textwidth]{figures/Power.eps}
%             \caption[]%
%             {{\small Network 3}}    
%             \label{fig:mean and std of net34}
%         \end{subfigure}
%         \hfill
%         \begin{subfigure}[b]{0.33\textwidth}   
%             \centering 
%             \includegraphics[width=\textwidth]{figures/Reward.eps}
%             \caption[]%
%             {{\small Network 4}}    
%             \label{fig:mean and std of net44}
%         \end{subfigure}
%         \caption[ The average and standard deviation of critical parameters ]
%         {\small The average and standard deviation of critical parameters: Region R4} 
%         \label{fig:mean and std of nets}
%     \end{figure*}
    
\begin{figure}[H]
     \centering
     \includegraphics[width=0.35\textwidth]{figures/Secrecy.eps}
     \caption{Secrecy.}
     %\vspace{-5mm}
     \label{fig:Secrecy}
 \end{figure}
